Bangladesh AI Readiness: Perspectives from the Academia, Industry, and Government

Artificial Intelligence (AI) readiness in the Global South extends beyond infrastructure to include curriculum design, workforce development, and cross-sector collaboration. Bangladesh, ranked 82nd in the 2023 Oxford Insights AI Readiness Index, exhibits significant deficits in technology capacity and research ecosystems, despite strong governmental visions. While HCI and ICTD research have explored digital inclusion and responsible AI, little empirical work examines how educational, industrial, and policy domains intersect to shape readiness. We present a multi-method qualitative study of AI readiness in Bangladesh, combining institutional analyses, 59 stakeholder interviews, and curriculum benchmarking against global exemplars. Findings reveal outdated curricula, limited faculty upskilling, inadequate computing resources, entrenched gender disparities, and the near-total absence of AI ethics instruction. We contribute empirical mapping of current practices, identification of structural and cultural barriers, and actionable pathways for embedding human-centered, inclusive, and responsible AI practices into national agendas, advancing equitable innovation in emerging AI ecosystems.

==> 0.0.updates.tex <==
1. intro -  SS wrote
2. lit -  
3. methods-  SS checked
4. context - SS checked
5. findings - SS working
6. discussion - 

Ela 
Tasmin
Mahzabin
Zinnat
Noman
Zulkarin
Mainul
Ishtiaque

==> 5.find.tex <==
%\clearpage
\section{Findings}

% blackboxing
% nested infrastructure
% strain
% path dependency

%%% material resource
%%% human resource and quality
%%% curriculum and beyond

This section presents the key insight from our surveys, interviews, focus group discussions and desktop research. It highlights the systemic gaps and limitations that currently inhibit effective AI readiness across Bangladeshi universities. Each subsection draws from observation notes, direct quotes from faculty and students, and institutional reviews, organized under five core areas.

\subsection{brought from methods}
The comparative matrix (see Table 2) highlights clear disparities between Bangladeshi programs and global best practices, especially in the areas of hands-on exposure to modern tools (e.g., LLMs, generative AI), integration of responsible AI, and real-world project work. This curriculum benchmarking further validated the qualitative insights collected through interviews, highlighting systemic misalignment between academic instruction and global AI workforce demands. 
Furthermore, our analysis extended to faculty and industry gender representation. Gender balance in AI departments and industry teams was found to be skewed, with male faculty and male-dominated teams prevalent in key AI fields across both academic and industrial sectors. This insight contributes to understanding the broader institutional and industrial dynamics that may affect AI education and workforce readiness in Bangladesh.


\subsection{Gaps in BD Academic Syllabus and Trendy AI Discourses}

Despite the rapid global evolution in AI, particularly in areas like Generative AI, Responsible AI, and interdisciplinary AI governance, most Bangladeshi universities remain anchored to outdated curricula that fail to align with modern trends and tools. While universities worldwide are quickly embracing hands-on learning environments, incorporating cutting-edge AI techniques such as Hugging Face models, RAG pipelines, AI ethics frameworks, and access to real-world datasets, many Bangladeshi institutions continue to follow traditional, theory-heavy syllabi designed before the AI revolution catalyzed by Large Language Models (LLMs) and diffusion models. This misalignment creates a significant gap between what students are learning in Bangladesh and the skills needed to excel in today's rapidly evolving AI industry.

Among the institutions surveyed, DU IIT stands out for offering a more structured set of courses that cover foundational AI, machine learning (ML), and image processing. However, even in DU IIT, there is no formal inclusion of trending topics such as Generative AI, LLMs, or Responsible AI in the curriculum, which means students are missing critical exposure to these important areas of study. On the other hand, universities like DU CSE, NSU, BUET, and BRACU offer only a limited number of AI courses, most of which are introduced in the final year, giving students little time to gain deep expertise in AI. Furthermore, the content remains heavily theoretical, focusing more on mathematical derivations rather than practical application and deployment of AI models.

As a result, students often end up learning about AI in isolation, without fully engaging with the tools and techniques that are transforming the field. For example, one student from X university described their experience as follows:

\begin{quote}
\textit{''During my undergrad at X university we covered the theoretical foundations of neural networks in depth, from activation functions to deriving the backpropagation algorithm by hand. But that was it. We never trained a model, never interacted with real datasets, and rarely used tools like TensorFlow or PyTorch. While we could explain the mathematics, we lacked the intuition that comes from seeing models learn and fail in practice.''} --- Student, X University
\end{quote}

This student's frustration speaks to the broader issue of AI education being disconnected from the real-world applications and cutting-edge technologies that are central to current AI research and employment needs. Without access to modern AI tools and the opportunity to work with real datasets, Bangladeshi students are left at a disadvantage, unable to develop the practical expertise needed to succeed in the AI-driven job market. 

This gap in the Bangladeshi AI curriculum is strongly echoed by professionals at the forefront of AI development in the country. According to industry experts, the expertise of fresh graduates from Bangladeshi universities often falls short of expectations. While students may possess a basic understanding of AI concepts, they lack exposure to critical and emerging areas such as Large Language Models (LLMs), Retrieval-Augmented Generation (RAG), and Responsible AI. Many industry professionals point out that students might technically know how to implement RAG pipelines, but they lack a deeper understanding of why such methods are needed, or what specific problems they are designed to solve. Their learning remains superficial, disconnected from real-world application and critical thinking. One of the senior member from a top multinational company at X Bangladesh says,


\begin{quote}
\textit{``I interviewed (for job) a student from one of the country's top public universities and asked, `Why use AI here? It can be solved in another way.' He couldn't answer. He knew the tools but not the reasoning behind them. That's where our curriculum is failing. Students aren't learning to solve real-world problems. Sure, you can connect four pieces of wood and call it a structure but unless they're aligned with purpose, it won't stand. Our AI education still revolves around outdated projects like chess bots, instead of tackling meaningful, real-world challenges. We're falling behind."} — Lead Engineer, X Company
\end{quote}


Industry leaders emphasize that curriculum reform must involve active participation from professionals in the field, alongside collaboration with international universities. Although such partnerships are often outlined in policy documents, they are rarely implemented in practice. This disconnect is attributed to a broader lack of engagement—both from academic faculty and from alumni currently working in industry—who could otherwise bridge the gap between academic instruction and real-world AI innovation. But a faculty member from X University acknowledged that staying aligned with industry developments remains a challenge:

\begin{quote}
\textit{``Unfortunately, we are not fully updated with the current trends in industry. This is partly due to a lack of interest from both sides and partly due to ego issues — industry often thinks academia does not understand practical constraints, while academia believes it is engaged in 'real' research. In other countries, collaborations are common, but here in Bangladesh they are rare. Even when both sides want to collaborate, factors like city traffic, long commute times, and workload make it difficult. We have revised our AI syllabus with industry feedback in the past two years, but guest lectures or hands-on training sessions from industry experts have become rare.''} --- Faculty Member, X University
\end{quote}



\input{5.tab-1}

Table 2 shows how Bangladeshi universities lag in the key dimensions of AI education when compared to top global programs. It clearly demonstrates the gaps between Bangladeshi universities and global institutions in the following areas:

\begin{itemize}
    \item \textbf{Human-Centered Mindset}: Bangladeshi universities rarely emphasize societal impacts or ethical considerations in AI.
    \item \textbf{Ethics of AI}: No dedicated course on AI ethics is offered at any Bangladeshi university.
    \item \textbf{AI Techniques and Applications}: There's a lack of hands-on exposure to advanced AI tools such as LLMs or Generative AI.
    \item \textbf{AI System Design}: Practical, real-world projects with industry collaboration are severely limited, meaning students miss out on crucial opportunities to apply their knowledge.
\end{itemize}

\subsection{Lack of Formal and Informal Training Opportunities for Faculty Members, Researchers, and Students}

Despite a growing national interest in AI, Bangladeshi universities lack a structured ecosystem to train and upskill faculty members, researchers, and students in AI methodologies and tools. There is no formal mechanism for continuous learning or professional development, leaving educators largely on their own to navigate the rapidly evolving AI landscape. This lack of institutional support for training and professional growth is evident in the research output of these universities. For example, BUET, which has the highest cumulative citation count of 21,768, still averages 1,281 citations per faculty, which, although respectable, is significantly lower compared to top global institutions. On the other hand, universities like BRACU, which has only 10,476 total citations, see a much lower average of 582 citations per faculty. This disparity highlights the impact that insufficient formal training and exposure to global AI communities can have on research productivity and the quality of scholarly work. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{output(2).png}
\caption{Bar chart showing Cumulative Citation Analysis of Total Citation vs Average Citation per faculty in AI/ML field in Bangladeshi Universities}
\label{fig:gender_chart}
\end{figure}

Across institutions, faculty rely heavily on self-study, free online courses, or occasional workshops—none of which are funded or recognized institutionally. This gap is particularly detrimental to early-career faculty, who often juggle heavy teaching loads with minimal time for research or skill development. Even at universities like NSU or BUET—known for their relatively stronger AI ecosystems—faculty development programs are missing. BRACU faculty design advanced AI courses but lack formal upskilling opportunities, and DU shows no explicit training either. One faculty member shared their frustration:

\begin{quote}
\textit{''I often try to keep my students updated with the latest trends in AI, but without formal training or opportunities to collaborate with global experts, there's a significant gap in what we can provide. The lack of institutional support for international exposure and ongoing professional development creates a barrier to advancing both faculty and student knowledge.''} --- Faculty, Y University
\end{quote}

On the student side, the situation is similarly challenging. While some research groups, hackathons, and mentorship programs exist, they are often inconsistent, limited in accessibility, and heavily reliant on a few passionate individuals. Access to these informal learning spaces is often based on connections, leading to exclusivity. Many students feel that they are unable to find mentorship or research opportunities within their own universities. As one student from Z University expressed:

\begin{quote}
\textit{''AI research groups exist, but access often depends on your connections and mostly on the basis of initial year's CGPA. If you don't have a high CGPA or you're not part of the right network, you can easily miss out on valuable learning opportunities, mentorship, and projects. It shouldn't be this way. AI should be accessible to anyone passionate about it, regardless of who they know.''} --- Student, Z University
\end{quote}

Beyond the university, students also face a significant lack of external opportunities for collaboration or mentorship. While a few companies, such as Samsung R\&D Bangladesh, offer mentorship and internship opportunities, such collaborations remain rare. Unfortunately, there are no structured or integrated systems for students to connect with other universities or companies for mentorship, internships, or research collaboration. Without these external avenues for learning and career development, students are left with minimal options for growth outside of the traditional classroom. As one student shared:

\begin{quote}
\textit{''I tried reaching out to teachers for advice or potential projects, but they were too busy or didn't have any ongoing research in AI. There are no clear pathways for internships or collaborations with other universities or companies, so it feels like there are no other options. You just have to hope you get lucky with the limited opportunities that come up.''} --- Student, X University
\end{quote}

The short academic semesters and the overemphasis on theoretical content leave little room for project incubation, hands-on practice, or collaborative learning environments. This lack of support for applied learning, combined with the absence of mentorship and guidance for research or career planning, contributes to a feeling of stagnation among students eager to pursue AI beyond the classroom.
When industry professionals were asked why stronger university-industry collaboration hasn't materialized, their response was strikingly candid. Many attributed the lack of engagement to a shared inertia on both sides:
\begin{quote}
\textit{''Honestly, it's not happening because no one is taking initiative. Faculty aren't reaching out, and engineers who came from these institutions aren't going back to help. Everyone's too comfortable in their own bubble.''} --- AI Engineer, Y Company
\end{quote}

According to multiple respondents, the responsibility lies with both the academic leadership and alumni working in the industry. Despite recognizing the need for change, little is being done to create sustainable channels for knowledge exchange, mentorship, or curriculum feedback.
\begin{quote}
\textit{''Universities have talented alumni working in AI globally. If even a few took the initiative to host regular seminars or guest lectures, students would be far more in tune with current industry trends. But right now, that kind of engagement is practically nonexistent.''} --- AI Engineer, Z Company
\end{quote}
This absence of proactive collaboration—from hosting industry talks to co-designing AI coursework—means that students often graduate with little exposure to how AI is actually practiced in modern industry settings. As one engineer remarked, the disconnect is less about capacity and more about accountability and motivation.

\subsection{Lack of Material, Software, and Hardware Resources}

The lack of access to GPUs is one of the most significant barriers in AI education in Bangladeshi universities. As AI research becomes increasingly complex, relying on personal laptops or low-performance hardware severely limits students' ability to work on advanced AI models and deploy real-world applications. Without access to high-performance computing infrastructure, the gap between students' learning and the current AI trends, like Generative AI, deep learning, and large language models widens.

In institutions like DU CSE or DU IIT, where GPU availability is minimal (only 2 GPUs for 148 students in DU IIT, or 5 GPUs for 240 students in DU CSE), only a small percentage of students can access the resources necessary to train deep learning models. This creates a situation where access to these resources often depends on factors like academic priority, faculty connections, or being involved in a funded thesis project. For most students, this means limited or no access to essential hardware and tools.

\begin{table*}[H]
\centering
\caption{Estimated GPU Availability and Student Population in AI-Focused Departments (2025)}
\begin{tabular}{|l|c|c|}
\hline
\textbf{University Department} & \textbf{Estimated Number of GPUs} & \textbf{Approx. Number of Students} \\
\hline
DU IIT & 2 & 148 \\
\hline
DU CSE & 5 & 240 \\
\hline
BUET CSE & 15--20 & 480 \\
\hline
BRACU CSE & 55 & 8,000 \\
\hline
NSU ECE & 39 & 6,000 \\
\hline
\end{tabular}
\label{tab:gpu_student_ratio}
\end{table*}

Table 3 illustrates the disparity between GPU availability and student population in Computer Science departments across Bangladeshi universities, highlighting the limited access to computational resources relative to the high number of students. This shortage in resources makes it extremely difficult for universities to coordinate the course curriculum. It not only restricts students' ability to build and deploy real-world AI projects, but also hinders their ability to stay updated with the latest developments in the field. AI research is progressing at an accelerated pace, and without modern infrastructure, students are forced to work with obsolete tools or rely on open-source alternatives that are not ideal for real-world applications. For instance, cloud credits (for platforms like Google Colab Pro, AWS Educate, or Microsoft Azure for Students) are crucial for modern AI workflows but are not provided by any university. One student from X University shared their frustration:

\begin{quote}
\textit{''I couldn't complete my project on time because I didn't have access to a decent system or enough storage to run models. It's frustrating when you have the theoretical knowledge but can't test or deploy it because the tools simply aren't available. It's a huge barrier, and it feels like we're being set up for failure when the infrastructure isn't there to support us.''} --- Student, X University
\end{quote}

A faculty member from X University echoed similar concerns, highlighting systemic issues that make it difficult to improve the situation:

\begin{quote}
\textit{''We don't have the funds to buy enough GPUs. AI is still comparatively new here, and the people in management who allocate funding are often not from computer science, so they don't fully understand why these resources are so critical. Space is another big problem — even though new buildings are being constructed, we haven't been allocated lab space. Politics plays a role too, older and more influential departments like social science or physics tend to get priority in funding and facilities, regardless of actual need. While top universities like IIT, NSU can provide decent internet and power backup, most of our PCs are too outdated to run modern deep learning models and would require a full upgrade. ''} --- Faculty Member, X University
\end{quote}

While BRACU and NSU reportedly have better lab setups, hardware usage remains exclusive and not integrated into standard coursework. Moreover, proprietary software such as MATLAB, SPSS, or annotation platforms is unavailable, making students dependent on limited open-source alternatives.

The inadequate availability of computational resources in Bangladeshi universities significantly hampers students' ability to engage with advanced AI technologies. This issue also extends into the professional world, where industry standards require familiarity with high-performance computing tools and platforms. A junior developer at Z Company, shared their frustration with a lack of real-world experience using GPUs, which impacted their ability to complete an AI proof of concept (PoC) within the timeline set by the company:

\begin{quote}
\textit{''I was assigned a task to develop an AI PoC for the company, but I couldn't meet the deadline because I had no experience working with GPUs in a real-world setting. I was used to working on personal laptops with minimal hardware, and when I tried running the models, the system couldn't handle the load. I ended up missing the project deadline, and the company had to bring in another developer with more experience. It was tough to get back on track.''} --- Junior AI Developer, Z Company
\end{quote}

Despite the growing demand for AI talent, most students and junior developers lack the infrastructure needed to succeed in real-world AI projects. The absence of paid cloud-based services, such as Google Cloud, AWS Educate, or Microsoft Azure for Students, which could provide them with access to cutting-edge resources and allow them to build more sophisticated models, further exacerbates this issue. Until universities and industries in Bangladesh begin to provide better access to these essential tools, students and developers will continue to face barriers in developing the necessary skills to succeed in the competitive global AI field.


\subsection{Lack of Norms and Opportunities for Cross-disciplinary and Cross-Sector Data Sharing and Collaboration}

While there is widespread recognition among Bangladeshi faculty of the transformative potential of interdisciplinary AI, universities in Bangladesh have yet to establish the structural frameworks needed to make such collaborations a reality. Currently, AI education and research remain largely confined within traditional departments like Computer Science and Engineering (CSE) or Electrical and Computer Engineering (ECE), with little to no integration into critical fields such as public health, agriculture, social sciences, or law. This siloed approach stifles the growth of AI applications that can have real-world impact, particularly in sectors that require the intersection of AI with domain-specific expertise.

In contrast, international universities like MIT, Stanford, and Oxford have embraced cross-disciplinary models that integrate AI into fields such as healthcare, environmental science, and sustainable development. For instance, Stanford University runs interdisciplinary programs like the Stanford AI for Social Good lab, which brings together experts from AI, social sciences, and public health to tackle global challenges. Similarly, MIT's Media Lab collaborates across disciplines, using AI to solve societal issues such as climate change, public health, and education. These global initiatives not only allow for better cross-sector collaboration but also provide students with a more holistic education, enabling them to apply AI to diverse, real-world problems.

However, in Bangladesh, the lack of formal platforms for collaboration keeps many faculty members and students isolated within their own departments. No joint courses, interdisciplinary thesis supervision, or collaborative labs exist that encourage faculty or students to work together across disciplines. As one faculty member from Z University expressed:

\begin{quote}
\textit{''Everyone recognizes the vast potential of applying AI across various fields, from healthcare to agriculture and social sciences, but there is no formal platform for collaboration. It's incredibly frustrating because while we all see the opportunities, the lack of institutional support and structured environments for interdisciplinary work keeps us stuck. ''} --- Faculty, Z University
\end{quote}
Moreover, faculty members at institutions like Y University struggle to connect with departments that have rich datasets but no way to collaborate with AI researchers. One faculty member from Y University shared:
\begin{quote}
\textit{''There are so many data-rich departments---like Botany or Environmental Science---that are working with field data, lab experiments, and seasonal datasets. But I don't even know they exist or how to access them. We have no forum for connecting with them, let alone doing AI-based research together.''} --- Faculty, Y University
\end{quote}
Another faculty member highlighted that beyond structural gaps, internal conflicts and departmental ego also hinder collaboration:
\begin{quote}
\textit{''Yes, there is internal conflict. For example, CSE people think we are the best and won't take help from Software Engineering, and Software Engineering people think they are the best. This kind of ego problem makes interdisciplinary work even harder, as departments are reluctant to share expertise or resources.''} --- Faculty, Z University
\end{quote}
The Bangladeshi academic landscape is therefore significantly lagging behind global counterparts in terms of creating interdisciplinary frameworks that promote cross-sector collaboration. Without these structures, Bangladesh risks falling behind in developing AI solutions that can solve complex, multi-faceted problems in areas like climate change, healthcare, and public policy, where AI's potential is most needed. In contrast, international institutions are already leading the way by fostering collaborations that bring AI expertise together with real-world applications in diverse fields.

\subsection{Gender Disparities}

Perhaps the most glaring structural imbalance observed in our study lies in gender representation within AI education and research in Bangladeshi universities. Faculty across all surveyed institutions are overwhelmingly male, with women holding only a small fraction of academic positions in AI-related departments. For instance, NSU's ECE department has only 3 female faculty out of 20, BRACU has 2 out of 18, BUET has 4 out of 17, and DU's CSE and IIT departments have no female AI faculty at all.

This imbalance contributes not only to the visibility gap but also to the absence of female mentors and role models in academic AI. As a result, female students often feel underrepresented and unsupported in their academic journey.

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{output(1).png}
\caption{Bar chart showing Gender Distribution of Faculty Engaged in AI Teaching and Research Across Major Bangladeshi Universities }
\label{fig:gender_chart}
\end{figure}

The issue extends beyond faculty statistics. Female students consistently reported subtle but impactful experiences of exclusion and bias. These included being overlooked in AI club leadership, sidelined during group projects, and discouraged from participating in research opportunities. In competitive spaces like final-year capstone projects, women often reported a need to overperform in order to receive the same recognition as their male counterparts.

\begin{quote}
\textit{``As a female student at Z University, I often feel like I have to prove myself twice as much during the capstone project selection process. Even when I take the lead and contribute significantly, the credit is often unfairly attributed to my male teammates. This not only undermines our efforts but also perpetuates the idea that women aren't as capable of taking charge in technical fields, despite the reality of our work and leadership.''} --- Female Student, Z University
\end{quote}

Such experiences, repeated across different campuses, indicate the presence of informal barriers to gender equity. The lack of inclusive policies, absence of gender-sensitive mentorship programs, and limited representation in institutional decision-making processes further marginalize women's participation in AI.

Students also noted that internship and research opportunities are often circulated informally through male-dominated networks. Consequently, women feel excluded not only from leadership but also from exposure to real-world experiences crucial to building a career in AI.

\begin{quote}
\textit{''Internship information usually spreads through boys' groups on WhatsApp. We're not always in those loops.''} --- Female Student, P University
\end{quote}

This unequal playing field has long-term consequences. Without intervention, it perpetuates the myth that AI is a male-dominated field, deterring future cohorts of women from entering or thriving in it. The lack of gender diversity also narrows the scope of AI solutions being developed—excluding perspectives that are vital for responsible and inclusive innovation.

In industry, the gender disparity is just as striking. The data on AI engineers across companies in Bangladesh shows that female representation remains significantly low. For instance, companies like Samsung, IQVIA, and others have minimal female representation in their AI teams, with female engineers accounting for only a small fraction of the workforce. This trend extends beyond academia, where the absence of women in key roles perpetuates the underrepresentation of female perspectives in the development of AI technologies. The chart below illustrates this disparity in gender distribution among AI engineers in various companies in Bangladesh.

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{output (6).png}
\caption{Gender Distribution of AI Engineers in Leading Bangladeshi Tech Companies}
\label{fig:industry_gender_chart}
\end{figure}

The low representation of female engineers in AI roles at major tech companies indicates a significant barrier to gender equity in the industry. This imbalance not only limits career opportunities for women but also hampers the development of AI solutions that are diverse and inclusive.

\subsection{Absence of Ethics and Responsible AI in Curricula}

One of the most concerning gaps in AI education across Bangladeshi universities is the complete absence of formal instruction on AI ethics, Responsible AI, or the social, legal, and ethical implications of AI systems. This lack of coverage is especially alarming as AI technologies increasingly influence critical sectors like healthcare, criminal justice, and finance, where the ethical implications can have far-reaching consequences. While some universities offer general philosophy or technology-society courses, none provide dedicated modules that focus specifically on the ethical concerns that arise when designing and deploying AI systems.

\begin{table*}[H]
\centering
\caption{AI Ethics Course Availability in Bangladeshi Universities (2025)}
\begin{tabular}{|l|l|l|}
\hline
\textbf{University} & \textbf{AI Ethics Course Offered} & \textbf{Remarks} \\
\hline
NSU (ECE) & General (PHI 104) & Covers broad ethics; no AI-specific content \\
\hline
BRACU (CSE) & General (HUM 347) & Discusses tech and society; lacks focus on AI \\
\hline
BUET (CSE) & None & No ethics or Responsible AI courses \\
\hline
DU (CSE) & None & No coverage of AI ethics, fairness, or safety \\
\hline
DU (IIT) & None & Entirely technical syllabus; ethics not mentioned \\
\hline
\end{tabular}
\end{table*}

The absence of AI ethics courses in the curricula is a direct result of the bureaucratic hurdles within the education system. In public universities, faculty members who wish to update or revise the syllabus face a long and tiring process involving approval from the University Grants Commission (UGC), a body whose leadership often consists of older members who may be unfamiliar with the rapid advancements in AI technologies and the emerging importance of ethics in AI. The UGC's outdated approach to curriculum development means that topics like AI ethics, fairness, and responsible AI are not prioritized or integrated into academic training, leaving Bangladeshi students at a disadvantage compared to their peers in other countries. As a faculty member from Z University explained, the process of updating the curriculum is often slow and frustrating, with many institutional hurdles:

\begin{quote}
\textit{''The process of changing the curriculum is incredibly time-consuming. You need multiple approvals from the UGC and the academic board, which means any proposed updates, especially those related to new topics like AI ethics, can take months—sometimes even years. By the time the curriculum is updated, it's often already outdated.''} --- Faculty, Z University
\end{quote}

Moreover, this systemic issue extends beyond the curriculum revision process. The lack of awareness among university decision-makers about the importance of AI ethics exacerbates the gap in AI education, as ethical concerns are often dismissed or treated as secondary to the technical skills required to build AI systems. Faculty members, despite their best efforts, are hindered by these structural and institutional barriers, which ultimately hinder the development of well-rounded, socially responsible AI professionals.

As one faculty member from Y University pointed out:
\begin{quote}
\textit{''We are teaching students how to build classifiers and models, but not how those models might reinforce bias or harm people. There's a huge disconnect between technical training and ethical considerations, and it's becoming harder to ignore as AI systems become more integrated into society.''} --- Faculty, Y University
\end{quote}

Students echoed similar concerns, often encountering ethical discussions only in social media or international webinars—not in their classrooms.

\begin{quote}
\textit{''I've never been taught about data privacy or fairness in any AI course. We just focus on math and code.''} --- Student, X University
\end{quote}

The lack of AI ethics education is a major barrier to creating responsible AI practitioners in Bangladesh. Without the proper foundation in ethical AI, students may graduate with technical skills but lack the understanding of how to apply those skills responsibly in real-world contexts.

This lack of focus on ethics in AI education is also evident in the industry. When asked if there was ever an incident where a junior developer neglected ethical considerations in AI and faced the consequences, a senior manager,  at Y company, reflected:

\begin{quote}
\textit{''Yes, actually — we had a junior developer once, fresh out of university, who built an essay scoring model for a government project. Technically, it was impressive. But he ignored fairness, used real student data without consent, and didn't think twice about explainability. The model ended up disadvantaging rural students and leaking personal info. It cost the company a major contract — and it cost him our trust. That's when we learned: in AI, ethical shortcuts always come with a price.''} —  Senior Manager, X Company.
\end{quote}

This example underscores the high cost of neglecting AI ethics in both academic training and professional practice. It serves as a critical reminder that the failure to incorporate responsible AI training can result in real-world consequences. As the demand for AI professionals grows, it is crucial that AI education in Bangladesh includes not only the technical skills but also the ethical foundation needed to ensure responsible and inclusive innovation.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> bibitems.tex <==
\begin{thebibliography}{9}

\bibitem{tbs2025chatgpt}
The Business Standard. \emph{AI policy draft written using ChatGPT, say experts}. (2025). Retrieved from \url{https://www.tbsnews.net/bangladesh/chatgpt-used-draft-bd-ai-policy-632182}

\bibitem{unesco2023aiethics}
UNESCO. \emph{Recommendation on the Ethics of Artificial Intelligence}. (2021). Retrieved from \url{https://unesdoc.unesco.org/ark:/48223/pf0000380455}

\bibitem{oecd2023trackingai}
OECD. \emph{OECD AI Policy Observatory: Tracking AI Implementation}. (2023). Retrieved from \url{https://oecd.ai}

\bibitem{ai-readiness-bd2025}
ICT Division and Startup Bangladesh. \emph{Glimpse of Bangladesh's AI Readiness}. (2025). Retrieved from \url{https://startupbangladesh.gov.bd}

\bibitem{sadat2023privacy}
Sarwat, Sadat and Sadat, Tawsif. \emph{Data Privacy and Protection in Bangladesh: 2023 Analysis}. (2023). Retrieved from \url{https://sadat-sarwat.com/data-privacy-bangladesh-2023-act/}

\bibitem{ai_strategy_2024}
Draft National AI Strategy of Bangladesh (2019–2024). ICT Division, Government of Bangladesh. \url{https://ictd.portal.gov.bd}

\bibitem{unescoethicsbd}
UNESCO Recommendation on the Ethics of Artificial Intelligence. \url{https://www.unesco.org/en/articles/advancing-ai-ethics-bangladesh}

\bibitem{privacybd2023}
Data Protection and Privacy Legislation in Bangladesh. UNCTAD. \url{https://unctad.org/page/data-protection-and-privacy-legislation-worldwide}

\bibitem{bgdcirt}
Bangladesh e-Gov Computer Incident Response Team. \url{https://www.cirt.gov.bd}

\bibitem{oxfordreadiness}
Oxford Insights AI Readiness Index (2023). \url{https://oxfordinsights.com/government-ai-readiness-index-2023}

\bibitem{worldbankregulatory}
World Bank Governance Indicators. \url{https://www.worldbank.org/en/publication/worldwide-governance-indicators}

\bibitem{gci2024}
Global Cybersecurity Index 5th Edition (2024). International Telecommunication Union. \url{https://www.itu.int/dms_pub/itu-d/opb/hdb/d-hdb-gci.01-2024-pdf-e.pdf}

\bibitem{egdi2024}
E-Government Development Index (2024), UN Public Administration Network. \url{https://publicadministration.un.org/egovkb/en-us/Data/Country-Information/id/14-Bangladesh}

\bibitem[14]{oxfordinsights2023}
Oxford Insights.
\newblock \emph{Government AI Readiness Index 2023}. 2023.
\newblock Available at: \url{https://oxfordinsights.com}.

\bibitem[15]{unesco2021ethics}
UNESCO.
\newblock \emph{Recommendation on the Ethics of Artificial Intelligence}. 2021.
\newblock Available at: \url{https://www.unesco.org}.

\bibitem[16]{euaiact2024}
Council of the European Union.
\newblock \emph{EU AI Act—Timeline and adoption (entry into force 2024)}. 2024.
\newblock Available at: \url{https://www.consilium.europa.eu}. See also: European Commission “AI Act” overview — \url{https://digital-strategy.ec.europa.eu} and \url{https://commission.europa.eu}.

\bibitem[17]{unescoAICF2025}
UNESCO.
\newblock \emph{AI Competency Framework for Students}. 2024/2025.
\newblock Available at: GCED Clearinghouse — \url{https://gcedclearinghouse.org}.

\bibitem[18]{aiedu2025}
aiEDU.
\newblock \emph{AI Readiness / AI Literacy \& Readiness Competencies}. 2024–2025.
\newblock Available at: \url{https://socialinnovationsjournal.com} and \url{https://aiedu.org} (Squarespace host).

\bibitem[19]{sambasivan2021fairnessIndia}
Sambasivan, N., et al.
\newblock “Re-imagining Algorithmic Fairness in India.” \emph{FAccT} 2021.
\newblock Available at: arXiv — \url{https://arxiv.org} and ACM Digital Library.

\bibitem[20]{sambasivan2021datawork}
Sambasivan, N., et al.
\newblock “Everyone wants to do the model work, not the data work.” \emph{CHI} 2021.
\newblock Available at: ACM Digital Library and SciSpace — \url{https://scispace.com}.

\bibitem[21]{kapania2022authority}
Kapania, S., et al.
\newblock “User Attitudes and Sources of AI Authority in India.” \emph{CHI} 2022.
\newblock Available at: ACM Digital Library — \url{https://dl.acm.org}.

\bibitem[22]{fu2024aiedu}
Fu, Y., et al.
\newblock “Navigating the ethical terrain of AI in education.” \emph{AIEDU (Cell Press)}, 2024 (review).
\newblock Available at: ScienceDirect — \url{https://www.sciencedirect.com}.

\bibitem[23]{dabis2024hepolicy}
Dabis, A., et al.
\newblock “AI and ethics: First policy responses of higher education.” \emph{Humanities \& Social Sciences Communications} (Nature), 2024.
\newblock Available at: \url{https://www.nature.com}.

\bibitem[24]{unesco2023less10}
UNESCO.
\newblock “Less than 10\% of schools/universities have formal AI guidance.” News brief, 2023 (updated 2024).
\newblock Available at: \url{https://www.unesco.org}.

\bibitem[25]{miaoHolmes2023}
Miao, F. and Holmes, W.
\newblock \emph{Guidance for Generative AI in Education and Research}. UNESCO, 2023.
\newblock Overview at: \url{https://www.unesco.org}.

\bibitem[26]{bdcsa2023}
People's Republic of Bangladesh.
\newblock \emph{Cyber Security Act, 2023}. Legislative text and analyses.
\newblock Available at: Refworld — \url{https://www.refworld.org} and Amnesty International — \url{https://www.amnesty.org}.

\bibitem[27]{bdpdp2025}
People's Republic of Bangladesh.
\newblock \emph{Draft Personal Data Protection Act (2023–2025 process)}. Analyses and timeline.
\newblock Available at: Transparency International Bangladesh — \url{https://www.ti-bangladesh.org} and Digital Policy Alert — \url{https://www.digitalpolicyalert.org}.

\end{thebibliography}


==> old-8.25.tex <==
\section{Methods}
Our mixed-method research involves interviews, surveys, and desktop research to investigate the state of AI readiness in Bangladesh, particularly across the academic, industrial, and governance sectors. Grounded in the aiEDU Readiness Framework and the UNESCO AI Competency Standards, our research aims to assess institutional capacity, curriculum adequacy, faculty development, infrastructure availability, and stakeholder engagement within key Bangladeshi universities. Furthermore, we explore how collaboration across academia, industry, and government currently functions and how it may be improved.
Our approach is multi-method and interpretive, combining structured institutional analysis with rich qualitative data from student and faculty interviews, two surveys, desktop research and stakeholder feedback from the industry.

% \textcolor{blue}{Note from Sharifa: We need a demographics table here (follow any of my published CHI or CSCW papers for this)}

\subsection{Participants Recruitment}

To capture the state of AI readiness and institutional collaboration dynamics in Bangladesh, we adopted a purposive sampling strategy, focusing on five prominent universities: BUET, DU (CSE and IIT), NSU, and BRACU. These institutions represent varying governance models (public vs. private), funding structures, and levels of access to infrastructure—conditions that are emblematic of broader educational asymmetries in the Global South.

We recruited 59 participants, comprising undergraduate and postgraduate students (n=25), faculty members (n=9), and industry professionals (n=25) working at or collaborating with these universities. Student and faculty participants were recruited via university mailing lists, social media, and peer referrals. Industry experts were identified through alumni networks and prior collaborative projects with academia.

This recruitment strategy was not aimed at statistical generalizability, but rather at capturing diverse, situated perspectives on AI education and collaboration practices in the Bangladeshi context.

\begin{table}[h]
\centering
\caption{Participant Demographics by Institution and Role}
\begin{tabular}{|l|l|c|c|c|}
\hline
\textbf{Participant Type} & \textbf{Institution/Org} & \textbf{Gender (M/F)} \\
\hline
\multirow{5}{*}{Undergraduate Students} 
  & BUET       & 5 (M:4; F:1)  \\
  & DU CSE     & 5 (M:3; F:2) \\
  & IIT DU     & 5 (M:3; F:2) \\
  & BRACU      & 5 (M:3; F:2) \\
  & NSU        & 5 (M:3; F:2) \\
\hline
\multirow{5}{*}{Faculty Members} 
  & BUET       & 2 (M:2; F:0) \\
  & DU CSE     & 2 (M:2; F:0) \\
  & IIT DU     & 2 (M:2; F:0) \\
  & BRACU      & 2 (M:2; F:0) \\
  & NSU        & 1 (M:1; F:0) \\
\hline
\multirow{5}{*}{Industry Professionals} 
  & Samsung R\&D BD     & 5 (M:4; F:1) \\
  & Streams Tech Ltd.   & 5 (M:5; F:0) \\
  & Cefalo              & 5 (M:4; F:1) \\
  & Factorize           & 5 (M:5; F:0) \\
  & Brain Station 23    & 5 (M:5; F:0) \\
\hline
\end{tabular}
\label{tab:demographics}
\end{table}

\subsection{One-on-One Interview}
We conducted one-on-one semi-structured interviews with students, educators, and professionals to understand their perceptions of AI education quality, institutional readiness, and cross-sector engagement. Interview protocols were informed by two internationally recognized frameworks: the \textit{aiEDU Readiness Framework}, which emphasizes curriculum, ethics, and infrastructure, and the \textit{UNESCO AI Competency Framework}, which foregrounds interdisciplinary and socially responsible AI education.

Student interviews explored the accessibility and relevance of AI coursework, perceived gaps in hands-on experience, mentorship availability, and awareness of ethical implications. Faculty interviews focused on curriculum design challenges, access to computing resources, and institutional support for AI pedagogy. Industry interviews probed expectations of AI graduates, experiences of academic collaboration, and barriers to offering internships or co-designed curricula.

Each interview lasted 45–60 minutes and was conducted in Bangla, as all of the participants preferred Bangla. All interviews were recorded, transcribed, and anonymized.


\subsection{Data Collection and Analysis}

We used a hybrid analytic approach combining inductive thematic coding with framework-informed analysis. Transcripts from interviews were independently open-coded by two researchers using grounded theory techniques. This inductive process allowed themes to emerge directly from participant narratives rather than imposing predefined categories. The emergent codes were then clustered into higher-level themes, guided by dimensions from the \textit{aiEDU Readiness Framework} and the \textit{UNESCO AI Competency Framework}, including: curriculum integration, educator competency, ethics and responsibility, infrastructural capacity, and stakeholder engagement.

To enhance validity and contextual depth, we triangulated these qualitative insights with document analysis of AI-related syllabus, course descriptions, faculty research profiles, and laboratory infrastructure descriptions collected from five Bangladeshi universities (BUET, DU CSE, DU IIT, BRACU, NSU). We also analyzed faculty citations, focusing on those in top AI conferences (e.g., NeurIPS, ICML, CVPR) and evaluated the number of faculty members actively publishing in these high-impact venues.

In addition to analyzing domestic academic materials, we conducted a structured comparative curriculum analysis between these five Bangladeshi universities and ten top-ranked global computer science programs (e.g., Stanford, MIT, CMU). This comparison was guided by the 2021 and 2025 UNESCO AI Competency Frameworks for Students, which define key AI learning dimensions such as human-centered mindset, ethics of AI, technical skill exposure, and AI system design. Each institution's curriculum was assessed along these axes through a coding rubric derived from UNESCO’s indicators.

Furthermore, our analysis extended to faculty and industry gender representation. We examined the gender ratio of faculty members teaching AI-related courses and evaluated the gender composition of AI industry teams across the universities. Gender balance in AI departments and industry teams was found to be skewed, with male faculty and male-dominated teams prevalent in key AI fields across both academic and industrial sectors. This insight contributes to understanding the broader institutional and industrial dynamics that may affect AI education and workforce readiness in Bangladesh.

We also conducted surveys to capture data on the availability of GPU resources and gender representation in AI teams. The first survey was circulated to university students to gauge access to GPUs for AI coursework, while the second survey was distributed to industry employees to assess the gender ratio within AI teams at prominent companies. These surveys revealed the disparity in resources and gender diversity across academic and industrial sectors, which was further explored in qualitative interviews.

The comparative matrix (see Table 2) highlights clear disparities between Bangladeshi programs and global best practices, especially in the areas of hands-on exposure to modern tools (e.g., LLMs, generative AI), integration of responsible AI, and real-world project work. This curriculum benchmarking further validated the qualitative insights collected through interviews, highlighting systemic misalignment between academic instruction and global AI workforce demands.

Coding disagreements between researchers were resolved through peer discussion. Thematic saturation was reached by the fifty-nine interviews, after which no substantially new themes were observed.

\subsection{Ethics and Positionality Statement}
All participants were briefed on the study’s goals and their rights, and informed consent was obtained prior to data collection.

As researchers embedded in Bangladeshi higher education and the AI research ecosystem, we bring both proximity and positional bias. Our own experiences with AI instruction, student mentorship, and policy advocacy influence how we interpret these findings. At the same time, this positionality granted access to restricted institutional documents and trust-based recruitment pathways that would be otherwise difficult to achieve.

We acknowledge the systemic inequalities that shape Global South research ecosystems, including underfunded public infrastructure, overreliance on donor priorities, and a growing but underrecognized innovation landscape. Our goal is not to universalize findings but to center local voices and institutional lived realities as valid forms of knowledge in global AI discourse.


\section{Findings}

% blackboxing
% nested infrastructure
% strain
% path dependency

%%% material resource
%%% human resource and quality
%%% curriculum and beyond

This section presents the key insight from our surveys, interviews, focus group discussions and desktop research. It highlights the systemic gaps and limitations that currently inhibit effective AI readiness across Bangladeshi universities. Each subsection draws from observation notes, direct quotes from faculty and students, and institutional reviews, organized under five core areas.

\subsection{brought from methods}
The comparative matrix (see Table 2) highlights clear disparities between Bangladeshi programs and global best practices, especially in the areas of hands-on exposure to modern tools (e.g., LLMs, generative AI), integration of responsible AI, and real-world project work. This curriculum benchmarking further validated the qualitative insights collected through interviews, highlighting systemic misalignment between academic instruction and global AI workforce demands. 
Furthermore, our analysis extended to faculty and industry gender representation. Gender balance in AI departments and industry teams was found to be skewed, with male faculty and male-dominated teams prevalent in key AI fields across both academic and industrial sectors. This insight contributes to understanding the broader institutional and industrial dynamics that may affect AI education and workforce readiness in Bangladesh.


\subsection{Gaps in BD Academic Syllabus and Trendy AI Discourses}

Despite the rapid global evolution in AI, particularly in areas like Generative AI, Responsible AI, and interdisciplinary AI governance, most Bangladeshi universities remain anchored to outdated curricula that fail to align with modern trends and tools. While universities worldwide are quickly embracing hands-on learning environments, incorporating cutting-edge AI techniques such as Hugging Face models, RAG pipelines, AI ethics frameworks, and access to real-world datasets, many Bangladeshi institutions continue to follow traditional, theory-heavy syllabi designed before the AI revolution catalyzed by Large Language Models (LLMs) and diffusion models. This misalignment creates a significant gap between what students are learning in Bangladesh and the skills needed to excel in today’s rapidly evolving AI industry.

Among the institutions surveyed, DU IIT stands out for offering a more structured set of courses that cover foundational AI, machine learning (ML), and image processing. However, even in DU IIT, there is no formal inclusion of trending topics such as Generative AI, LLMs, or Responsible AI in the curriculum, which means students are missing critical exposure to these important areas of study. On the other hand, universities like DU CSE, NSU, BUET, and BRACU offer only a limited number of AI courses, most of which are introduced in the final year, giving students little time to gain deep expertise in AI. Furthermore, the content remains heavily theoretical, focusing more on mathematical derivations rather than practical application and deployment of AI models.

As a result, students often end up learning about AI in isolation, without fully engaging with the tools and techniques that are transforming the field. For example, one student from X university described their experience as follows:

\begin{quote}
\textit{''During my undergrad at X university we covered the theoretical foundations of neural networks in depth, from activation functions to deriving the backpropagation algorithm by hand. But that was it. We never trained a model, never interacted with real datasets, and rarely used tools like TensorFlow or PyTorch. While we could explain the mathematics, we lacked the intuition that comes from seeing models learn and fail in practice.''} --- Student, X University
\end{quote}

This student’s frustration speaks to the broader issue of AI education being disconnected from the real-world applications and cutting-edge technologies that are central to current AI research and employment needs. Without access to modern AI tools and the opportunity to work with real datasets, Bangladeshi students are left at a disadvantage, unable to develop the practical expertise needed to succeed in the AI-driven job market. 

This gap in the Bangladeshi AI curriculum is strongly echoed by professionals at the forefront of AI development in the country. According to industry experts, the expertise of fresh graduates from Bangladeshi universities often falls short of expectations. While students may possess a basic understanding of AI concepts, they lack exposure to critical and emerging areas such as Large Language Models (LLMs), Retrieval-Augmented Generation (RAG), and Responsible AI. Many industry professionals point out that students might technically know how to implement RAG pipelines, but they lack a deeper understanding of why such methods are needed, or what specific problems they are designed to solve. Their learning remains superficial, disconnected from real-world application and critical thinking. One of the senior member from a top multinational company at X Bangladesh says,


\begin{quote}
\textit{“I interviewed a student from one of the country’s top public universities and asked, ‘Why use AI here? It can be solved in another way.’ He couldn’t answer. He knew the tools but not the reasoning behind them. That’s where our curriculum is failing. Students aren’t learning to solve real-world problems. Sure, you can connect four pieces of wood and call it a structure but unless they’re aligned with purpose, it won’t stand. Our AI education still revolves around outdated projects like chess bots, instead of tackling meaningful, real-world challenges. We’re falling behind.”} — Lead Engineer, X Company
\end{quote}


Industry leaders emphasize that curriculum reform must involve active participation from professionals in the field, alongside collaboration with international universities. Although such partnerships are often outlined in policy documents, they are rarely implemented in practice. This disconnect is attributed to a broader lack of engagement—both from academic faculty and from alumni currently working in industry—who could otherwise bridge the gap between academic instruction and real-world AI innovation. But a faculty member from X University acknowledged that staying aligned with industry developments remains a challenge:

\begin{quote}
\textit{``Unfortunately we are not fully updated with the current trends in industry. This is partly due to a lack of interest from both sides and partly due to ego issues — industry often thinks academia does not understand practical constraints, while academia believes it is engaged in 'real' research. In other countries, collaborations are common, but here in Bangladesh they are rare. Even when both sides want to collaborate, factors like city traffic, long commute times, and workload make it difficult. We have revised our AI syllabus with industry feedback in the past two years, but guest lectures or hands-on training sessions from industry experts have become rare.''} --- Faculty Member, X University
\end{quote}



\input{5.tab-1}

Table 2 shows how Bangladeshi universities lag in the key dimensions of AI education when compared to top global programs. It clearly demonstrates the gaps between Bangladeshi universities and global institutions in the following areas:

\begin{itemize}
    \item \textbf{Human-Centered Mindset}: Bangladeshi universities rarely emphasize societal impacts or ethical considerations in AI.
    \item \textbf{Ethics of AI}: No dedicated course on AI ethics is offered at any Bangladeshi university.
    \item \textbf{AI Techniques and Applications}: There’s a lack of hands-on exposure to advanced AI tools such as LLMs or Generative AI.
    \item \textbf{AI System Design}: Practical, real-world projects with industry collaboration are severely limited, meaning students miss out on crucial opportunities to apply their knowledge.
\end{itemize}

\subsection{Lack of Formal and Informal Training Opportunities for Faculty Members, Researchers, and Students}

Despite a growing national interest in AI, Bangladeshi universities lack a structured ecosystem to train and upskill faculty members, researchers, and students in AI methodologies and tools. There is no formal mechanism for continuous learning or professional development, leaving educators largely on their own to navigate the rapidly evolving AI landscape. This lack of institutional support for training and professional growth is evident in the research output of these universities. For example, BUET, which has the highest cumulative citation count of 21,768, still averages 1,281 citations per faculty, which, although respectable, is significantly lower compared to top global institutions. On the other hand, universities like BRACU, which has only 10,476 total citations, see a much lower average of 582 citations per faculty. This disparity highlights the impact that insufficient formal training and exposure to global AI communities can have on research productivity and the quality of scholarly work. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{output(2).png}
\caption{Bar chart showing Cumulative Citation Analysis of Total Citation vs Average Citation per faculty in AI/ML field in Bangladeshi Universities}
\label{fig:gender_chart}
\end{figure}

Across institutions, faculty rely heavily on self-study, free online courses, or occasional workshops—none of which are funded or recognized institutionally. This gap is particularly detrimental to early-career faculty, who often juggle heavy teaching loads with minimal time for research or skill development. Even at universities like NSU or BUET—known for their relatively stronger AI ecosystems—faculty development programs are missing. BRACU faculty design advanced AI courses but lack formal upskilling opportunities, and DU shows no explicit training either. One faculty member shared their frustration:

\begin{quote}
\textit{''I often try to keep my students updated with the latest trends in AI, but without formal training or opportunities to collaborate with global experts, there's a significant gap in what we can provide. The lack of institutional support for international exposure and ongoing professional development creates a barrier to advancing both faculty and student knowledge.''} --- Faculty, Y University
\end{quote}

On the student side, the situation is similarly challenging. While some research groups, hackathons, and mentorship programs exist, they are often inconsistent, limited in accessibility, and heavily reliant on a few passionate individuals. Access to these informal learning spaces is often based on connections, leading to exclusivity. Many students feel that they are unable to find mentorship or research opportunities within their own universities. As one student from Z University expressed:

\begin{quote}
\textit{''AI research groups exist, but access often depends on your connections and mostly on the basis of initial year's CGPA. If you don't have a high CGPA or you're not part of the right network, you can easily miss out on valuable learning opportunities, mentorship, and projects. It shouldn't be this way. AI should be accessible to anyone passionate about it, regardless of who they know.''} --- Student, Z University
\end{quote}

Beyond the university, students also face a significant lack of external opportunities for collaboration or mentorship. While a few companies, such as Samsung R\&D Bangladesh, offer mentorship and internship opportunities, such collaborations remain rare. Unfortunately, there are no structured or integrated systems for students to connect with other universities or companies for mentorship, internships, or research collaboration. Without these external avenues for learning and career development, students are left with minimal options for growth outside of the traditional classroom. As one student shared:

\begin{quote}
\textit{''I tried reaching out to teachers for advice or potential projects, but they were too busy or didn’t have any ongoing research in AI. There are no clear pathways for internships or collaborations with other universities or companies, so it feels like there are no other options. You just have to hope you get lucky with the limited opportunities that come up.''} --- Student, X University
\end{quote}

The short academic semesters and the overemphasis on theoretical content leave little room for project incubation, hands-on practice, or collaborative learning environments. This lack of support for applied learning, combined with the absence of mentorship and guidance for research or career planning, contributes to a feeling of stagnation among students eager to pursue AI beyond the classroom.
When industry professionals were asked why stronger university-industry collaboration hasn’t materialized, their response was strikingly candid. Many attributed the lack of engagement to a shared inertia on both sides:
\begin{quote}
\textit{''Honestly, it’s not happening because no one is taking initiative. Faculty aren’t reaching out, and engineers who came from these institutions aren’t going back to help. Everyone’s too comfortable in their own bubble.''} --- AI Engineer, Y Company
\end{quote}

According to multiple respondents, the responsibility lies with both the academic leadership and alumni working in the industry. Despite recognizing the need for change, little is being done to create sustainable channels for knowledge exchange, mentorship, or curriculum feedback.
\begin{quote}
\textit{''Universities have talented alumni working in AI globally. If even a few took the initiative to host regular seminars or guest lectures, students would be far more in tune with current industry trends. But right now, that kind of engagement is practically nonexistent.''} --- AI Engineer, Z Company
\end{quote}
This absence of proactive collaboration—from hosting industry talks to co-designing AI coursework—means that students often graduate with little exposure to how AI is actually practiced in modern industry settings. As one engineer remarked, the disconnect is less about capacity and more about accountability and motivation.

\subsection{Lack of Material, Software, and Hardware Resources}

The lack of access to GPUs is one of the most significant barriers in AI education in Bangladeshi universities. As AI research becomes increasingly complex, relying on personal laptops or low-performance hardware severely limits students' ability to work on advanced AI models and deploy real-world applications. Without access to high-performance computing infrastructure, the gap between students’ learning and the current AI trends, like Generative AI, deep learning, and large language models widens.

In institutions like DU CSE or DU IIT, where GPU availability is minimal (only 2 GPUs for 148 students in DU IIT, or 5 GPUs for 240 students in DU CSE), only a small percentage of students can access the resources necessary to train deep learning models. This creates a situation where access to these resources often depends on factors like academic priority, faculty connections, or being involved in a funded thesis project. For most students, this means limited or no access to essential hardware and tools.

\begin{table*}[H]
\centering
\caption{Estimated GPU Availability and Student Population in AI-Focused Departments (2025)}
\begin{tabular}{|l|c|c|}
\hline
\textbf{University Department} & \textbf{Estimated Number of GPUs} & \textbf{Approx. Number of Students} \\
\hline
DU IIT & 2 & 148 \\
\hline
DU CSE & 5 & 240 \\
\hline
BUET CSE & 15--20 & 480 \\
\hline
BRACU CSE & 55 & 8,000 \\
\hline
NSU ECE & 39 & 6,000 \\
\hline
\end{tabular}
\label{tab:gpu_student_ratio}
\end{table*}

Table 3 illustrates the disparity between GPU availability and student population in Computer Science departments across Bangladeshi universities, highlighting the limited access to computational resources relative to the high number of students. This shortage in resources makes it extremely difficult for universities to coordinate the course curriculum. It not only restricts students' ability to build and deploy real-world AI projects, but also hinders their ability to stay updated with the latest developments in the field. AI research is progressing at an accelerated pace, and without modern infrastructure, students are forced to work with obsolete tools or rely on open-source alternatives that are not ideal for real-world applications. For instance, cloud credits (for platforms like Google Colab Pro, AWS Educate, or Microsoft Azure for Students) are crucial for modern AI workflows but are not provided by any university. One student from X University shared their frustration:

\begin{quote}
\textit{''I couldn’t complete my project on time because I didn’t have access to a decent system or enough storage to run models. It’s frustrating when you have the theoretical knowledge but can’t test or deploy it because the tools simply aren’t available. It’s a huge barrier, and it feels like we’re being set up for failure when the infrastructure isn’t there to support us.''} --- Student, X University
\end{quote}

A faculty member from X University echoed similar concerns, highlighting systemic issues that make it difficult to improve the situation:

\begin{quote}
\textit{''We don’t have the funds to buy enough GPUs. AI is still comparatively new here, and the people in management who allocate funding are often not from computer science, so they don’t fully understand why these resources are so critical. Space is another big problem — even though new buildings are being constructed, we haven’t been allocated lab space. Politics plays a role too, older and more influential departments like social science or physics tend to get priority in funding and facilities, regardless of actual need. While top universities like IIT, NSU can provide decent internet and power backup, most of our PCs are too outdated to run modern deep learning models and would require a full upgrade. ''} --- Faculty Member, X University
\end{quote}

While BRACU and NSU reportedly have better lab setups, hardware usage remains exclusive and not integrated into standard coursework. Moreover, proprietary software such as MATLAB, SPSS, or annotation platforms is unavailable, making students dependent on limited open-source alternatives.

The inadequate availability of computational resources in Bangladeshi universities significantly hampers students' ability to engage with advanced AI technologies. This issue also extends into the professional world, where industry standards require familiarity with high-performance computing tools and platforms. A junior developer at Z Company, shared their frustration with a lack of real-world experience using GPUs, which impacted their ability to complete an AI proof of concept (PoC) within the timeline set by the company:

\begin{quote}
\textit{''I was assigned a task to develop an AI PoC for the company, but I couldn’t meet the deadline because I had no experience working with GPUs in a real-world setting. I was used to working on personal laptops with minimal hardware, and when I tried running the models, the system couldn’t handle the load. I ended up missing the project deadline, and the company had to bring in another developer with more experience. It was tough to get back on track.''} --- Junior AI Developer, Z Company
\end{quote}

Despite the growing demand for AI talent, most students and junior developers lack the infrastructure needed to succeed in real-world AI projects. The absence of paid cloud-based services, such as Google Cloud, AWS Educate, or Microsoft Azure for Students, which could provide them with access to cutting-edge resources and allow them to build more sophisticated models, further exacerbates this issue. Until universities and industries in Bangladesh begin to provide better access to these essential tools, students and developers will continue to face barriers in developing the necessary skills to succeed in the competitive global AI field.


\subsection{Lack of Norms and Opportunities for Cross-disciplinary and Cross-Sector Data Sharing and Collaboration}

While there is widespread recognition among Bangladeshi faculty of the transformative potential of interdisciplinary AI, universities in Bangladesh have yet to establish the structural frameworks needed to make such collaborations a reality. Currently, AI education and research remain largely confined within traditional departments like Computer Science and Engineering (CSE) or Electrical and Computer Engineering (ECE), with little to no integration into critical fields such as public health, agriculture, social sciences, or law. This siloed approach stifles the growth of AI applications that can have real-world impact, particularly in sectors that require the intersection of AI with domain-specific expertise.

In contrast, international universities like MIT, Stanford, and Oxford have embraced cross-disciplinary models that integrate AI into fields such as healthcare, environmental science, and sustainable development. For instance, Stanford University runs interdisciplinary programs like the Stanford AI for Social Good lab, which brings together experts from AI, social sciences, and public health to tackle global challenges. Similarly, MIT's Media Lab collaborates across disciplines, using AI to solve societal issues such as climate change, public health, and education. These global initiatives not only allow for better cross-sector collaboration but also provide students with a more holistic education, enabling them to apply AI to diverse, real-world problems.

However, in Bangladesh, the lack of formal platforms for collaboration keeps many faculty members and students isolated within their own departments. No joint courses, interdisciplinary thesis supervision, or collaborative labs exist that encourage faculty or students to work together across disciplines. As one faculty member from Z University expressed:

\begin{quote}
\textit{''Everyone recognizes the vast potential of applying AI across various fields, from healthcare to agriculture and social sciences, but there is no formal platform for collaboration. It’s incredibly frustrating because while we all see the opportunities, the lack of institutional support and structured environments for interdisciplinary work keeps us stuck. ''} --- Faculty, Z University
\end{quote}
Moreover, faculty members at institutions like Y University struggle to connect with departments that have rich datasets but no way to collaborate with AI researchers. One faculty member from Y University shared:
\begin{quote}
\textit{''There are so many data-rich departments---like Botany or Environmental Science---that are working with field data, lab experiments, and seasonal datasets. But I don’t even know they exist or how to access them. We have no forum for connecting with them, let alone doing AI-based research together.''} --- Faculty, Y University
\end{quote}
Another faculty member highlighted that beyond structural gaps, internal conflicts and departmental ego also hinder collaboration:
\begin{quote}
\textit{''Yes, there is internal conflict. For example, CSE people think we are the best and won’t take help from Software Engineering, and Software Engineering people think they are the best. This kind of ego problem makes interdisciplinary work even harder, as departments are reluctant to share expertise or resources.''} --- Faculty, Z University
\end{quote}
The Bangladeshi academic landscape is therefore significantly lagging behind global counterparts in terms of creating interdisciplinary frameworks that promote cross-sector collaboration. Without these structures, Bangladesh risks falling behind in developing AI solutions that can solve complex, multi-faceted problems in areas like climate change, healthcare, and public policy, where AI’s potential is most needed. In contrast, international institutions are already leading the way by fostering collaborations that bring AI expertise together with real-world applications in diverse fields.

\subsection{Gender Disparities}

Perhaps the most glaring structural imbalance observed in our study lies in gender representation within AI education and research in Bangladeshi universities. Faculty across all surveyed institutions are overwhelmingly male, with women holding only a small fraction of academic positions in AI-related departments. For instance, NSU's ECE department has only 3 female faculty out of 20, BRACU has 2 out of 18, BUET has 4 out of 17, and DU’s CSE and IIT departments have no female AI faculty at all.

This imbalance contributes not only to the visibility gap but also to the absence of female mentors and role models in academic AI. As a result, female students often feel underrepresented and unsupported in their academic journey.

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{output(1).png}
\caption{Bar chart showing Gender Distribution of Faculty Engaged in AI Teaching and Research Across Major Bangladeshi Universities }
\label{fig:gender_chart}
\end{figure}

The issue extends beyond faculty statistics. Female students consistently reported subtle but impactful experiences of exclusion and bias. These included being overlooked in AI club leadership, sidelined during group projects, and discouraged from participating in research opportunities. In competitive spaces like final-year capstone projects, women often reported a need to overperform in order to receive the same recognition as their male counterparts.

\begin{quote}
\textit{``As a female student at Z University, I often feel like I have to prove myself twice as much during the capstone project selection process. Even when I take the lead and contribute significantly, the credit is often unfairly attributed to my male teammates. This not only undermines our efforts but also perpetuates the idea that women aren’t as capable of taking charge in technical fields, despite the reality of our work and leadership.''} --- Female Student, Z University
\end{quote}

Such experiences, repeated across different campuses, indicate the presence of informal barriers to gender equity. The lack of inclusive policies, absence of gender-sensitive mentorship programs, and limited representation in institutional decision-making processes further marginalize women’s participation in AI.

Students also noted that internship and research opportunities are often circulated informally through male-dominated networks. Consequently, women feel excluded not only from leadership but also from exposure to real-world experiences crucial to building a career in AI.

\begin{quote}
\textit{''Internship information usually spreads through boys’ groups on WhatsApp. We’re not always in those loops.''} --- Female Student, P University
\end{quote}

This unequal playing field has long-term consequences. Without intervention, it perpetuates the myth that AI is a male-dominated field, deterring future cohorts of women from entering or thriving in it. The lack of gender diversity also narrows the scope of AI solutions being developed—excluding perspectives that are vital for responsible and inclusive innovation.

In industry, the gender disparity is just as striking. The data on AI engineers across companies in Bangladesh shows that female representation remains significantly low. For instance, companies like Samsung, IQVIA, and others have minimal female representation in their AI teams, with female engineers accounting for only a small fraction of the workforce. This trend extends beyond academia, where the absence of women in key roles perpetuates the underrepresentation of female perspectives in the development of AI technologies. The chart below illustrates this disparity in gender distribution among AI engineers in various companies in Bangladesh.

\begin{figure}[!t]
\centering
\includegraphics[width=0.7\columnwidth]{output (6).png}
\caption{Gender Distribution of AI Engineers in Leading Bangladeshi Tech Companies}
\label{fig:industry_gender_chart}
\end{figure}

The low representation of female engineers in AI roles at major tech companies indicates a significant barrier to gender equity in the industry. This imbalance not only limits career opportunities for women but also hampers the development of AI solutions that are diverse and inclusive.

\subsection{Absence of Ethics and Responsible AI in Curricula}

One of the most concerning gaps in AI education across Bangladeshi universities is the complete absence of formal instruction on AI ethics, Responsible AI, or the social, legal, and ethical implications of AI systems. This lack of coverage is especially alarming as AI technologies increasingly influence critical sectors like healthcare, criminal justice, and finance, where the ethical implications can have far-reaching consequences. While some universities offer general philosophy or technology-society courses, none provide dedicated modules that focus specifically on the ethical concerns that arise when designing and deploying AI systems.

\begin{table*}[H]
\centering
\caption{AI Ethics Course Availability in Bangladeshi Universities (2025)}
\begin{tabular}{|l|l|l|}
\hline
\textbf{University} & \textbf{AI Ethics Course Offered} & \textbf{Remarks} \\
\hline
NSU (ECE) & General (PHI 104) & Covers broad ethics; no AI-specific content \\
\hline
BRACU (CSE) & General (HUM 347) & Discusses tech and society; lacks focus on AI \\
\hline
BUET (CSE) & None & No ethics or Responsible AI courses \\
\hline
DU (CSE) & None & No coverage of AI ethics, fairness, or safety \\
\hline
DU (IIT) & None & Entirely technical syllabus; ethics not mentioned \\
\hline
\end{tabular}
\end{table*}

The absence of AI ethics courses in the curricula is a direct result of the bureaucratic hurdles within the education system. In public universities, faculty members who wish to update or revise the syllabus face a long and tiring process involving approval from the University Grants Commission (UGC), a body whose leadership often consists of older members who may be unfamiliar with the rapid advancements in AI technologies and the emerging importance of ethics in AI. The UGC’s outdated approach to curriculum development means that topics like AI ethics, fairness, and responsible AI are not prioritized or integrated into academic training, leaving Bangladeshi students at a disadvantage compared to their peers in other countries. As a faculty member from Z University explained, the process of updating the curriculum is often slow and frustrating, with many institutional hurdles:

\begin{quote}
\textit{''The process of changing the curriculum is incredibly time-consuming. You need multiple approvals from the UGC and the academic board, which means any proposed updates, especially those related to new topics like AI ethics, can take months—sometimes even years. By the time the curriculum is updated, it’s often already outdated.''} --- Faculty, Z University
\end{quote}

Moreover, this systemic issue extends beyond the curriculum revision process. The lack of awareness among university decision-makers about the importance of AI ethics exacerbates the gap in AI education, as ethical concerns are often dismissed or treated as secondary to the technical skills required to build AI systems. Faculty members, despite their best efforts, are hindered by these structural and institutional barriers, which ultimately hinder the development of well-rounded, socially responsible AI professionals.

As one faculty member from Y University pointed out:
\begin{quote}
\textit{''We are teaching students how to build classifiers and models, but not how those models might reinforce bias or harm people. There’s a huge disconnect between technical training and ethical considerations, and it's becoming harder to ignore as AI systems become more integrated into society.''} --- Faculty, Y University
\end{quote}

Students echoed similar concerns, often encountering ethical discussions only in social media or international webinars—not in their classrooms.

\begin{quote}
\textit{''I've never been taught about data privacy or fairness in any AI course. We just focus on math and code.''} --- Student, X University
\end{quote}

The lack of AI ethics education is a major barrier to creating responsible AI practitioners in Bangladesh. Without the proper foundation in ethical AI, students may graduate with technical skills but lack the understanding of how to apply those skills responsibly in real-world contexts.

This lack of focus on ethics in AI education is also evident in the industry. When asked if there was ever an incident where a junior developer neglected ethical considerations in AI and faced the consequences, a senior manager,  at Y company, reflected:

\begin{quote}
\textit{''Yes, actually — we had a junior developer once, fresh out of university, who built an essay scoring model for a government project. Technically, it was impressive. But he ignored fairness, used real student data without consent, and didn’t think twice about explainability. The model ended up disadvantaging rural students and leaking personal info. It cost the company a major contract — and it cost him our trust. That’s when we learned: in AI, ethical shortcuts always come with a price.''} —  Senior Manager, X Company.
\end{quote}

This example underscores the high cost of neglecting AI ethics in both academic training and professional practice. It serves as a critical reminder that the failure to incorporate responsible AI training can result in real-world consequences. As the demand for AI professionals grows, it is crucial that AI education in Bangladesh includes not only the technical skills but also the ethical foundation needed to ensure responsible and inclusive innovation.


==> tab-1.tex <==
\begin{table}[!t]
\begin{center}
\begin{tabular}{|rl|}
\hline
Total Participants: & 41 (Female: 24, Male: 17)\\
\hdashline
\multicolumn{2}{|c|}{\textbf{Type of Participation}} \\
\hdashline
Interview only: & 8 (Female: 5, Male: 3)\\
FGD only: & 15 (Female: 8, Male: 7)\\
Interview + FGD: & 18 (Female: 11, Male: 7)\\
\hdashline

\multicolumn{2}{|c|}{\textbf{Age range (in Years)}} \\
\hdashline
All: & 19-60, median 33\\
Female: & 19-60, median 30\\
Male: & 19-56, median 38\\
\hdashline

\multicolumn{2}{|c|}{\textbf{Family Income Range (per month, in USD)}} \\
\hdashline
All: & 50-500, median 100  \\
Female: & 80-200, median 94  \\
Male: & 50-500, median 85  \\
\hdashline

\multicolumn{2}{|c|}{\textbf{Education}} \\
\hdashline
No Formal Schooling: & 15 (Female: 8, Male: 7)\\
Primary School: & 18 (Female: 10, Male: 8)\\
Secondary School: & 5 (Female: 3, Male: 2)\\
Higher Secondary School: & 2 (Female: 2, Male: 0)\\
Undergraduate and Above: & 1 (Female: 1, Male: 0)\\
\hline

\end{tabular}
\end{center}
\caption{Details of the Participants}
\end{table}






==> table1-full.tex <==
\begin{table*}[t]
\begin{center}
 \begin{tabular}{|C{1.3cm}| R{1.5cm}  L{0.5cm} | R{3.0cm}  L{0.5cm} | R{4.0cm}  L{0.3cm} |}
 \hline
\multicolumn{7}{|c|}{\multirow{2}{*}{\textbf{Details of Pre-Design Survey, Interviews, and Focus Group Discussions}}}\\ 
\multicolumn{7}{|c|}{} \\ \hline
 
 \multirow{6}{*}{Survey} & \multicolumn{6}{c|}{\textbf{Total Number of Survey Responses: 321 (Female: 211, Male: 110)}}\\ \cline{2-7}
  & \multicolumn{2}{c}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{|c|}{\textbf{Type of Incidents}} & 
 \multicolumn{2}{|c|}{\textbf{Other Details}} \\ \cline{2-7} 
& 18-20:  &  52    &   Molestation:                &   267    &                              &   \\
& 21-25:  &  221   &   Exhibiting Private Part:    &   53     &   Parent of Victim:              &   21 \\
& 26-30:  &  36    &   Rape/Attempt:               &   48     &   Victim Received Medical Aid:   & 14  \\
& 31-35:  &  5     &   Force showing Pron:         &   22     &   Victim Received legal  Aid:    &   2 \\
& 36-40:  &  4     &   Forcing to Undress:         &   21     &                              &   \\
& 41+:    &  3     &   Other:                      &   4      &                              &   \\ \hline
 
\hline
 
\multirow{ 6}{*}{Interview} & \multicolumn{6}{c|}{\textbf{Total Number of Interview Participants: 20 (Female:16, Male:4)}}\\ \cline{2-7}
& \multicolumn{2}{c}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{|c|}{\textbf{Occupation}} & 
 \multicolumn{2}{|c|}{\textbf{Other Details}} \\ \cline{2-7}
& 18-20:  &  0    &   Educator:     &   7    &                              &   \\
& 21-25:  &  0    &   Housewife:    &   6    &   Parents:                   & 15  \\
& 26-30:  &  4    &   NGO Worker:   &   2    &   Were Themselves Victim:    &  6 \\
& 31-35:  &  11   &   Doctor:       &   1    &   In Touch with Children:    &  20 \\
& 36-40:  &  2    &   Student:      &   0    &                              &   \\
& 41+:    &  3    &   Other:        &   4    &                              &   \\ \hline

\multirow{ 6}{*}{FGD} & \multicolumn{6}{c|}{\textbf{Total Number of FGD Participants: 20 (Female:14, Male:6)}}\\ \cline{2-7}
& \multicolumn{2}{c}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{|c|}{\textbf{Occupation}} & 
 \multicolumn{2}{|c|}{\textbf{Other Details}} \\ \cline{2-7}
& 18-20:  &   1    &   Educator:     &   1    &            &   \\
& 21-25:  &   12   &   Housewife:    &   2    &   Parents:                 &  8  \\
& 26-30:  &  2     &   NGO Worker:   &   1    &   Were Themselves Victim:  &  6  \\
& 31-35:  &  4     &   Doctor:       &   2    &   In Touch With Children:  &  20  \\
& 36-40:  &  0     &   Student:      &   5    &            &   \\
& 41+:    &  2     &   Other:        &   9    &             &   \\ \hline

\end{tabular}
\end{center}
\caption{Details of the Survey, Interview, and FGD Participants}
\end{table*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}

\begin{table}
\begin{center}
 \begin{tabular}{|R{3cm}  L{3cm} | R{3cm}  L{3cm} |}
 \hline
 \multicolumn{4}{|c|}{\textbf{Total Participation: 91}}\\ \hdashline
 \multicolumn{2}{|c|}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{c|}{\textbf{Occupation}} \\ \hdashline
18-25:  &   52 (57\%)   &   Student:    &   53 (58\%)\\
26-35:  &   36 (40\%)   &   Public/Private Employee:    &   27 (29\%)\\
36-45: &     2 (2\%) &   Teacher:    &   5 (6\%)\\
46+: &     1 (1\%) &   Others:    &   6 (7\%)\\ \hdashline
 
 \multicolumn{2}{|c|}{\textbf{Relation with Harasser}} &
 \multicolumn{2}{c|}{\textbf{Victims Action Towards Legal Steps}} \\ \hdashline
 
  Relatives:  &   11 (9\%)   &   Ignorant of Legal Steps:    &   8 (9\%)\\
  Stranger: &     72 (58\%) &   Parents are Reluctant:    &   9 (10\%)\\

 Friends:  &   34 (28\%)   &   No:    &  70 (77\%)\\
Others: &     6 (5\%) &   Yes:    &   1 (1\%) \\
 &     &   Others:    &   3 (3\%) \\ \hdashline
 

\multicolumn{4}{|c|}{\textbf{Form of Harassment}} \\ \hdashline

\multicolumn{2}{|r}{Cursing and sending vulgar texts:}    &  \multicolumn{2}{l|}{68 (38\%)}\\
\multicolumn{2}{|r}{Repetitively asking to date/marry:}    &  \multicolumn{2}{l|}{39 (22\%)}\\
\multicolumn{2}{|r}{Sending images of private bodyparts:}    &  \multicolumn{2}{l|}{24 (13\%)}\\
\multicolumn{2}{|r}{Requesting nude photos:}    &  \multicolumn{2}{l|}{14 (8\%)}\\
\multicolumn{2}{|r}{Threatening with fabricated  pornographic photos:}    &  \multicolumn{2}{l|}{9 (5\%)}\\
\multicolumn{2}{|r}{Threatening to kidnap, rape, and murder:}    &  \multicolumn{2}{l|}{7 (4\%)}\\
\multicolumn{2}{|r}{Others:}    &  \multicolumn{2}{l|}{18 (10\%)}\\
\hline
 
\end{tabular}
\end{center}
\caption{Demographic Characteristics of the Survey Participants}
\end{table}

\end{comment}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table}
\begin{center}
 \begin{tabular}{|R{3cm}  L{3cm} | R{3cm}  L{3cm} |}
 \hline
 \multicolumn{4}{|c|}{\textbf{Total Participation: 91}}\\ \hdashline
 \multicolumn{2}{|c|}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{c|}{\textbf{Occupation}} \\ \hdashline
18-25:  &   52 (57\%)   &   Student:    &   53 (58\%)\\
26-35:  &   36 (40\%)   &   Public/Private Employee:    &   27 (29\%)\\
36-45: &     2 (2\%) &   Teacher:    &   5 (6\%)\\
46+: &     1 (1\%) &   Others:    &   6 (7\%)\\ \hline

\end{tabular}
\end{center}
\caption{Demographic Characteristics of the Survey Participants}
\end{table}
\end{comment}

==> table1.tex <==
\begin{table*}[t]
\begin{center}
 \begin{tabular}{|C{1.3cm}| R{1.5cm}  L{0.5cm} | R{3.0cm}  L{0.5cm} | R{4.0cm}  L{0.3cm} |}
 \hline
\multicolumn{7}{|c|}{\multirow{2}{*}{\textbf{Details of Pre-Design Survey}}}\\ 
\multicolumn{7}{|c|}{} \\ \hline
 
 \multirow{6}{*}{Survey} & \multicolumn{6}{c|}{\textbf{Total Number of Survey Responses: 321 (Female: 211, Male: 110)}}\\ \cline{2-7}
  & \multicolumn{2}{c}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{|c|}{\textbf{Type of Incidents}} & 
 \multicolumn{2}{|c|}{\textbf{Other Details}} \\ \cline{2-7} 
& 18-20:  &  52    &   Molestation:                &   267    &                              &   \\
& 21-25:  &  221   &   Exhibiting Private Part:    &   53     &   Parent of Victim:              &   21 \\
& 26-30:  &  36    &   Rape/Attempt:               &   48     &   Victim Received Medical Aid:   & 14  \\
& 31-35:  &  5     &   Force showing \newedits{Porn}:         &   22     &   Victim Received legal  Aid:    &   2 \\
& 36-40:  &  4     &   Forcing to Undress:         &   21     &                              &   \\
& 41+:    &  3     &   Other:                      &   4      &                              &   \\ \hline
 
\hline
 
\end{tabular}
\end{center}
\caption{Details of the Survey Participants}
\end{table*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}

\begin{table}
\begin{center}
 \begin{tabular}{|R{3cm}  L{3cm} | R{3cm}  L{3cm} |}
 \hline
 \multicolumn{4}{|c|}{\textbf{Total Participation: 91}}\\ \hdashline
 \multicolumn{2}{|c|}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{c|}{\textbf{Occupation}} \\ \hdashline
18-25:  &   52 (57\%)   &   Student:    &   53 (58\%)\\
26-35:  &   36 (40\%)   &   Public/Private Employee:    &   27 (29\%)\\
36-45: &     2 (2\%) &   Teacher:    &   5 (6\%)\\
46+: &     1 (1\%) &   Others:    &   6 (7\%)\\ \hdashline
 
 \multicolumn{2}{|c|}{\textbf{Relation with Harasser}} &
 \multicolumn{2}{c|}{\textbf{Victims Action Towards Legal Steps}} \\ \hdashline
 
  Relatives:  &   11 (9\%)   &   Ignorant of Legal Steps:    &   8 (9\%)\\
  Stranger: &     72 (58\%) &   Parents are Reluctant:    &   9 (10\%)\\

 Friends:  &   34 (28\%)   &   No:    &  70 (77\%)\\
Others: &     6 (5\%) &   Yes:    &   1 (1\%) \\
 &     &   Others:    &   3 (3\%) \\ \hdashline
 

\multicolumn{4}{|c|}{\textbf{Form of Harassment}} \\ \hdashline

\multicolumn{2}{|r}{Cursing and sending vulgar texts:}    &  \multicolumn{2}{l|}{68 (38\%)}\\
\multicolumn{2}{|r}{Repetitively asking to date/marry:}    &  \multicolumn{2}{l|}{39 (22\%)}\\
\multicolumn{2}{|r}{Sending images of private bodyparts:}    &  \multicolumn{2}{l|}{24 (13\%)}\\
\multicolumn{2}{|r}{Requesting nude photos:}    &  \multicolumn{2}{l|}{14 (8\%)}\\
\multicolumn{2}{|r}{Threatening with fabricated  pornographic photos:}    &  \multicolumn{2}{l|}{9 (5\%)}\\
\multicolumn{2}{|r}{Threatening to kidnap, rape, and murder:}    &  \multicolumn{2}{l|}{7 (4\%)}\\
\multicolumn{2}{|r}{Others:}    &  \multicolumn{2}{l|}{18 (10\%)}\\
\hline
 
\end{tabular}
\end{center}
\caption{Demographic Characteristics of the Survey Participants}
\end{table}

\end{comment}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table}
\begin{center}
 \begin{tabular}{|R{3cm}  L{3cm} | R{3cm}  L{3cm} |}
 \hline
 \multicolumn{4}{|c|}{\textbf{Total Participation: 91}}\\ \hdashline
 \multicolumn{2}{|c|}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{c|}{\textbf{Occupation}} \\ \hdashline
18-25:  &   52 (57\%)   &   Student:    &   53 (58\%)\\
26-35:  &   36 (40\%)   &   Public/Private Employee:    &   27 (29\%)\\
36-45: &     2 (2\%) &   Teacher:    &   5 (6\%)\\
46+: &     1 (1\%) &   Others:    &   6 (7\%)\\ \hline

\end{tabular}
\end{center}
\caption{Demographic Characteristics of the Survey Participants}
\end{table}
\end{comment}

==> table2.tex <==
\begin{table*}[t]
\begin{center}
 \begin{tabular}{|C{1.3cm}| R{1.5cm}  L{0.5cm} | R{2.0cm}  L{0.5cm} | R{3.5cm}  L{0.3cm} |}
 \hline
\multicolumn{7}{|c|}{\multirow{2}{*}{\textbf{Details of Post-Design Feedback Interviews and Focus Group Discussions}}}\\ 
\multicolumn{7}{|c|}{} \\ \hline

 
\multirow{ 6}{*}{Interview} & \multicolumn{6}{c|}{\textbf{Number of Interview Sessions and Participants: 20 (Female:16, Male:4)}}\\ \cline{2-7}
& \multicolumn{2}{c}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{|c|}{\textbf{Occupation}} & 
 \multicolumn{2}{|c|}{\textbf{Other Details}} \\ \cline{2-7}
& 18-20:  &  0    &   Educator:     &   7    &                              &   \\
& 21-25:  &  0    &   Housewife:    &   6    &   Parents:                   & 15  \\
& 26-30:  &  4    &   NGO Worker:   &   2    &   Were Themselves Victim:    &  6 \\
& 31-35:  &  11   &   Doctor:       &   1    &   In Touch with Children:    & 20  \\
& 36-40:  &  2    &   Student:      &   0    &                              &   \\
& 41+:    &  3    &   Other:        &   4    &                              &   \\ \hline


\multirow{ 6}{*}{FGD} & \multicolumn{6}{c|}{\textbf{Number of FGD Sessions: 7; Number of Participants: 26 (Female:13, Male:13)}}\\ \cline{2-7}
& \multicolumn{2}{c}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{|c|}{\textbf{Occupation}} & 
 \multicolumn{2}{|c|}{\textbf{Other Details)}} \\ \cline{2-7}
& 18-20:  &   1   &   Educator:     &    1   &             &   \\
& 21-25:  &   19  &   Housewife:    &    2   &   Parents:          & 4  \\
& 26-30:  &   2   &   NGO Worker:   &    0   &   Were Themselves Victim:   & 7  \\
& 31-35:  &   2   &   Doctor:       &    2   &   In Touch with Children:  &  26 \\
& 36-40:  &   0   &   Student:      &    10  &            &   \\
& 41+:    &   2   &   Other:        &    11  &             &   \\ \hline

\end{tabular}
\end{center}
\caption{Demographic Characteristics of Post-Design Interview and Focus Group Discussion Participants}
\end{table*}

==> table3.tex <==
\begin{table*}[t]
\begin{center}
 \begin{tabular}{|C{1.3cm}| R{1.5cm}  L{0.5cm} | R{2.0cm}  L{0.5cm} | R{3.5cm}  L{0.3cm} |}
 \hline
\multicolumn{7}{|c|}{\multirow{2}{*}{\textbf{Details of Pre-Design Interviews and Focus Group Discussions}}}\\ 
\multicolumn{7}{|c|}{} \\ \hline

\multirow{ 6}{*}{Interview} & \multicolumn{6}{c|}{\textbf{Number of Interview Sessions and Participants: 20 (Female: 16, Male: 4)}}\\ \cline{2-7}
& \multicolumn{2}{c}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{|c|}{\textbf{Occupation}} & 
 \multicolumn{2}{|c|}{\textbf{Other Details}} \\ \cline{2-7}
& 18-20:  &  0    &   Educator:     &   7    &                              &   \\
& 21-25:  &  0    &   Housewife:    &   6    &   Parents:                   & 15  \\
& 26-30:  &  4    &   NGO Worker:   &   2    &   Were Themselves Victim:    &  6 \\
& 31-35:  &  11   &   Doctor:       &   1    &   In Touch with Children:    &  20 \\
& 36-40:  &  2    &   Student:      &   0    &                              &   \\
& 41+:    &  3    &   Other:        &   4    &                              &   \\ \hline

\multirow{ 6}{*}{FGD} & \multicolumn{6}{c|}{\textbf{Number of FGD Sessions: 5; Number of Participants: 20 (Female: 14, Male: 6)}}\\ \cline{2-7}
& \multicolumn{2}{c}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{|c|}{\textbf{Occupation}} & 
 \multicolumn{2}{|c|}{\textbf{Other Details}} \\ \cline{2-7}
& 18-20:  &   1    &   Educator:     &   1    &            &   \\
& 21-25:  &   12   &   Housewife:    &   2    &   Parents:                 &  8  \\
& 26-30:  &  2     &   NGO Worker:   &   1    &   Were Themselves Victim:  &  6  \\
& 31-35:  &  4     &   Doctor:       &   2    &   In Touch With Children:  &  20  \\
& 36-40:  &  0     &   Student:      &   5    &            &   \\
& 41+:    &  2     &   Other:        &   9    &             &   \\ \hline

\end{tabular}
\end{center}
\caption{Demographic Details of Interview and FGD Participants}
\end{table*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}

\begin{table}
\begin{center}
 \begin{tabular}{|R{3cm}  L{3cm} | R{3cm}  L{3cm} |}
 \hline
 \multicolumn{4}{|c|}{\textbf{Total Participation: 91}}\\ \hdashline
 \multicolumn{2}{|c|}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{c|}{\textbf{Occupation}} \\ \hdashline
18-25:  &   52 (57\%)   &   Student:    &   53 (58\%)\\
26-35:  &   36 (40\%)   &   Public/Private Employee:    &   27 (29\%)\\
36-45: &     2 (2\%) &   Teacher:    &   5 (6\%)\\
46+: &     1 (1\%) &   Others:    &   6 (7\%)\\ \hdashline
 
 \multicolumn{2}{|c|}{\textbf{Relation with Harasser}} &
 \multicolumn{2}{c|}{\textbf{Victims Action Towards Legal Steps}} \\ \hdashline
 
  Relatives:  &   11 (9\%)   &   Ignorant of Legal Steps:    &   8 (9\%)\\
  Stranger: &     72 (58\%) &   Parents are Reluctant:    &   9 (10\%)\\

 Friends:  &   34 (28\%)   &   No:    &  70 (77\%)\\
Others: &     6 (5\%) &   Yes:    &   1 (1\%) \\
 &     &   Others:    &   3 (3\%) \\ \hdashline
 

\multicolumn{4}{|c|}{\textbf{Form of Harassment}} \\ \hdashline

\multicolumn{2}{|r}{Cursing and sending vulgar texts:}    &  \multicolumn{2}{l|}{68 (38\%)}\\
\multicolumn{2}{|r}{Repetitively asking to date/marry:}    &  \multicolumn{2}{l|}{39 (22\%)}\\
\multicolumn{2}{|r}{Sending images of private bodyparts:}    &  \multicolumn{2}{l|}{24 (13\%)}\\
\multicolumn{2}{|r}{Requesting nude photos:}    &  \multicolumn{2}{l|}{14 (8\%)}\\
\multicolumn{2}{|r}{Threatening with fabricated  pornographic photos:}    &  \multicolumn{2}{l|}{9 (5\%)}\\
\multicolumn{2}{|r}{Threatening to kidnap, rape, and murder:}    &  \multicolumn{2}{l|}{7 (4\%)}\\
\multicolumn{2}{|r}{Others:}    &  \multicolumn{2}{l|}{18 (10\%)}\\
\hline
 
\end{tabular}
\end{center}
\caption{Demographic Characteristics of the Survey Participants}
\end{table}

\end{comment}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table}
\begin{center}
 \begin{tabular}{|R{3cm}  L{3cm} | R{3cm}  L{3cm} |}
 \hline
 \multicolumn{4}{|c|}{\textbf{Total Participation: 91}}\\ \hdashline
 \multicolumn{2}{|c|}{\textbf{Age Range (in Years)}} &
 \multicolumn{2}{c|}{\textbf{Occupation}} \\ \hdashline
18-25:  &   52 (57\%)   &   Student:    &   53 (58\%)\\
26-35:  &   36 (40\%)   &   Public/Private Employee:    &   27 (29\%)\\
36-45: &     2 (2\%) &   Teacher:    &   5 (6\%)\\
46+: &     1 (1\%) &   Others:    &   6 (7\%)\\ \hline

\end{tabular}
\end{center}
\caption{Demographic Characteristics of the Survey Participants}
\end{table}
\end{comment}
